Tensor Factorization via Matrix Factorization

Tensor factorization arises in many machine learning applications, such knowledge base modeling and parameter estimation in latent variable models. However, numerical methods for tensor factorization have not reached the level of maturity of matrix factorization methods. In this paper, we propose a new method for CP tensor factorization that uses random projections to reduce the problem to simultaneous matrix diagonalization. Our method is conceptually simple and also applies to non-orthogonal and asymmetric tensors of arbitrary order. We prove that a small number random projections essentially preserves the spectral information in the tensor, allowing us to remove the dependence on the eigengap that plagued earlier tensor-to-matrix reductions. Experimentally, our method outperforms existing tensor factorization methods on both simulated data and two real datasets.

==> convergence.tex <==
\section{Convergence of the orthogonal tensor factorization method: empirical analysis}
\label{sec:convergence}

\begin{center}
\begin{figure}
\includegraphics[width=18cm]{figures/histogram.eps} \label{fig:histogram}
\caption{Histogram of objective values attained by the Jacobi simultaneous diagonalization algorithm for 1000 random sets of jointly diagonalizable matrices initialized with various amounts of noise.}
\end{figure}
\end{center}

To assess the convergence properties of the Jacobi method, we ran the algorithm
1000 times on different sets of $k$ random matrices ($k=d=15$) corrupted with
varying amounts of noise ($\e = 0,1e-4, 1e-3$). At each run, we measured the
objective value function (the Frobenius norm of the off-diagonal elements), and
plotted the resulting histogram (Figure \ref{fig:histogram}).

Overall, we observe that the objective values for a Gaussian distribution for
the three settings $\e = 0, 1e-4, 1e-3$. All data points are concentrated in an
interval that depend either on the convergence threshold ($1e-12$) in the
$\e=0$ case or on the noise level (when $\e=1e-3,1e-4$). Most interestingly,
when $\e=0$, the mean of the observations is around $1e-10$ (which corresponds
to the precision of $1e-12$ multiplied by the $\sim$ 200 entries in the
matrices), and $\e>0$, the mean depends on the noise level. Quite strikingly,
multiplying the noise by ten produces essentially the same histogram within the
same bounds, except that it has been translated from between 0.035 and 0.045 to
between 0.35 and 0.45.

This observation strongly suggests that the Jacobi algorithm attains a globally
optimal solutions for even small \pl{large?} values of noise.
\pl{But the experiments also demonstrate cases where it doesn't converge to the
global optimum...}

\begin{center}
\begin{figure}
\includegraphics[width=18cm]{figures/ojd-vs-als.eps} \label{fig:ojd-vs-als}
\caption{Comparing OJD vs ALS on random tensors.}
\end{figure}
\end{center}

As an example of how local optima can affect a solution, and to better contrast the performance of our method, we constructed artificial tensors $(d=k=5)$ in a way analogous to how we constructed matrices above. We compared our orthogonal OJD algorithm to alternating least squares (ALS), a method that is known to suffer from local optima. Results appear in Figure \ref{fig:ojd-vs-als}. Whereas the OJD accuracies are comparable to the noise level, many ALS results are completely inaccurate.

\begin{center}
\begin{figure}
\includegraphics[width=18cm]{figures/nojd-histogram.eps} \label{fig:nojd-histogram}
\caption{Histogram of objective values attained by the QRJ1D algorithm for 1000 random sets of jointly diagonalizable matrices initialized with various amounts of noise.}
\end{figure}
\end{center}

We also repeated the same experiments in the non-orthogonal setting using the QRJ1D algorithm. We plot the results in Figure \ref{fig:nojd-histogram}. Unlike the Jacobi method, QRJ1D clearly suffers from local optima in general.

\begin{center}
\begin{figure}
\includegraphics[width=18cm]{figures/nojd-small-mu.eps} \label{fig:nojd-small-mu}
\caption{Histogram of objective values attained by the QRJ1D algorithm for 1000 random sets of jointly diagonalizable matrices initialized with various amounts of noise.}
\end{figure}
\end{center}

However, these maxima only affect matrices with bad incoherence values. Repeating the experiment on matrices satisfying our incoherence assumption $\mu < 1/2d$ yielded the results in Figure \ref{fig:nojd-small-mu}. These results are quite similar to the orthogonal case.


==> extn-proof.tex <==
\section{Proofs for extensions}

\subsection{Asymmetric tensors}

\subsection{Higher-order tensors}
\label{app:higher-order-proofs}

Collapse tensor into a third-order tensor with one dimension being very large. This increases $\mu$ by a factor of $p$ (this is only linear compared to others, for whom it is exponential!).



==> initialization.tex <==
\section{Initialization}
\label{sec:initialization}

\pl{what is this section about?}

What happens with good restarts

Behavior with random restarts

Several iterations guaranteed to do well



==> ortho-pert-lemma.tex <==
\section{Convergence of the orthogonal tensor factorization method: formal analysis}
\label{sec:ortho-pert-lemma}

\pl{I'd remove this from this paper and save it for when we actually
understand the global convergence properties better;
it's a waste to have this buried in Appendix K;
it should probably be its own note;
one might argue the same for Appendix J}

In this section, we analyze the convergence of the Jacobi method. We argue that
for small enough $\e > 0$, Jacobi will converge to a point at which our
perturbation lemma holds. The results in this section complement our empirical
assessment of the convergence of the method.

\subsection{Notation}
Let $F(V, \sM) : O(n) \to \mathbb R^+$ be the orthogonal joint diagonalization criterion for a set of matrices $\sM = \{M_1, \cdots, M_L\}$,
\begin{align*}
  F(V, \sM) 
    &= \sum_{i=1}^L \| \off(V^\top M_l V) \|_F^2 \\
    &= \sum_{i=1}^L \| V^\top M_l V \|_F^2 - \| \diag(V^\top M_l V) \|_F^2.
\end{align*}

Let $\sM_\epsilon = \{ U^\top D_l U + \epsilon R_l \}_{l=1}^{L}$ be the
set of matrices given as input. Note that when $\epsilon = 0$, the set
of matrices commute and are jointly diagonalizable, with diagonalizer
$U$. For simplicity, we will let the set of matrices $U^\top D_l U$ be fixed and use the shorthand $F(V,\e)$ to denote $F(V, \sM_\e)$.

Several observations should be made about $F(V, \e)$:
\begin{itemize}
\item $F(V, \e)$ is continuous in $V, \e$. Since $O(n)$ is compact, for any fixed $\e$, $F(V, \e)$ is uniformly continuous.
\item If we restrict $\e$ to lie on a closed interval $I$, then $F(V, \e) : O(n) \times I \to \mathbb R^+$ is uniformly continuous with both variables and with the metric $|| \cdot ||'$ on $(V,\e)$ defined as $ || (V,\e) ||' = || V || + |\e| $.
\item Each global minimizer $U$ of $F(V, 0)$ is isolated. We let $\gamma > 0$ denote the radius of the ball
$$ \Gamma := \{V : || V - U || < \gamma \} $$
around $U$ on which $F(V,0) > F(U,0)$ for all $V \in \Gamma$.
\end{itemize}

Finally we introduce a few additional pieces of notation. We let $V(\e)$  minimizers of $F(V,\e)$ on the set $\Gamma$; such minimizers always exist by compactness of $F(V,\e)$. We also define $U(\e)$ to be a global minimizer of $F(V,\e)$; note that $U(0) = U$. Let $d(V)$ denote the Jacobi step taken from $V$: if $V^+ = \textrm{Jacobi}(V)$, then $d(V) = (V^+ - V)$. Finally, let $W(\e)$ to be the joint diagonalizer obtained from diagonalizing a single matrix in $\sM_\e$.

\subsection{Outline}

Our goal is to show that if Jacobi is initialized with $W(\e)$, then all sufficiently small $\e$, it will will converge to a point at which Cardoso's lemma holds. This involves several steps:
\begin{enumerate}
\item Showing that Jacobi converges to a point close to an unperturbed local minimum $U$.
\item For all such points that are close to $U$, Cardoso's lemma holds.
\end{enumerate}

\subsection{Convergence of Jacobi to a neighborhood of $U$}

Our first lemma states that the steps taken by Jacobi get arbitrarily small when the objective value is close to optimal.

\begin{lemma}[Vanishing steps]
\label{lem:d_k-bound}
Let $U(\e)$ be a global minimizer of $F(V,\e)$. For all $\delta > 0$, there is a $t > 0$ such for all $\e > 0$, whenever $| F(U(\e), \e) - F(V,\e) | < t$, $|| d(V) || < \delta$.
\end{lemma}

\begin{proof}
Follows from some algebra (see Maleko, 2003).
%Let $c_{ij} = \left( (M_l)_{ij} \right)_{l=1}^L$ be the vector of the $i,j$-th value across all the diagonalized matrices. For any fixed $i,j$, define
%\begin{align*}
%A &= || c_{ij} ||^2 \\
%B &= || c_{jj} - c_{ii} ||^2 \\
%C &= c_{ij}^T (c_{jj} - c_{ii})
%\end{align*}
%Also, let 
%$$ S(\theta) = \sum_{l=1}^L \left( G(\theta,i,j)^T M_l G(\theta,i,j) \right)_{ij}^2 $$
%be the sum of the squared $i,j$-th off diagonal elements after the matrices have been rotated by a Givens rotation matrix $G(\theta, i,j)$.
%
%One can show using some algebra that 
%$$ S(\theta, A, B, C) = \frac{A-B/4}{2} \cos4\theta + \frac{A+B/4}{2} + \frac{C}{2} \sin4\theta. $$
%If $| F(U(\e), \e) - F(V,\e) | < t$, then the maximal reduction $| S(\theta) - S(0) |$ is less than $t$. Since Jacobi only decreases $S(\theta)$.
%
%Since the function $S(\theta, A, B, C)$ is continuous and each of its variables are bounded, it is also uniformly continuous. Hence, there is a ball $|\theta| \leq \theta_0$ such that for all $A,B,C$, $ | S(\theta, A,B,C) - S(0,A,B,C) | < t$. Since $S$ is injective in $\theta$ on $[0,\pi/2]$, this must
\end{proof}

Next, we want to establish local convergence results for Jacobi: when it is started close to a local minimizer, it converges to that minimizer. 

First, we will need to show that the step sizes Jacobi takes are small around certain local minimizers of $F(V,\e)$. In particular, when a local minimizer $V(\e)$ is close to $U$, we can use the fact that the steps around $U$ are small to show that steps around $V$ are small as well. This is what the following lemma establishes.

\begin{lemma}[Vanishing steps around local minima]
\label{lem:convergence-threshold}
For all $\gamma > \delta > 0$, there exists an $\e_0 > 0$ and an $r > 0$ such that for all $0 \leq \e \leq \e_0$, if $ V(\e) $ is a minimizer of $F(V,\e)$ on the set $\Gamma = \{V : | V - U | \leq \gamma\}$ satisfying  $ || U - V(\e) || < r $, then we have
$$ || V - V(\e) || + || d(V) || < \delta $$
whenever $|| V - V(\e) || < r$.
\end{lemma}

\begin{proof}
By \lemmaref{d_k-bound}, there exists a $t > 0$ such that for any $\e \geq 0$, $| F(U(\e), \e) - F(V,\e) | < t$ implies that $|| d(V) || < \delta / 2$.

Choose $r > 0$ such that $r < \delta /2 $ and such that for all $|| V - U || < 2r$, we have $| F(U(0), 0) - F(V,0) | < t/4$.
Choose $\e_0 > 0$  such that for all $V \in O(n)$ and all $0 \leq \e \leq \e_0$, we have $ || F(V,0) - F(V,\e) || < t/4. $
%Choose $\e_1 > 0$  such that for $0 \leq \e \leq \e_1$, we have $ || F(U(0),0) - F(U(\e),0) || < t/4. $

Then, when $|| V - V(\e) || < r$, we have $|| V - U || \leq || V - V(\e) || + || V(\e) - U || \leq 2r$, and thus $| F(U(0), 0) - F(V,0) | < t/4$.

Next, for $0 \leq \e \leq \e_0$, and for the same $V$ as above we have
\begin{align*}
F(V,\e) - F(U(\e), \e)
%& = F(V,\e) - F(V,0) + F(V,0) - F(U(\e), \e) + F(U(\e), 0) - F(U(\e), 0) \\
%& \;\;\;\;\;\; + F(U(0), 0) - F(U(0), 0) \\
& \leq | F(V, \e) - F(V,0) | + | F(U(\e), \e) - F(U(\e), 0) | \\
& \;\;\;\;\;\; + | F(U(0), 0) - F(U(\e), 0) | + | F(V,0) - F(U(0), 0) | \\
& < t / 4 + t / 4 + t / 4 + t / 4
= t.
\end{align*}
By definition of $t$, $|| d(V) || < \delta / 2 $ and
$$ || V - V(\e) || + || d(V) || < \delta /2 + \delta /2 \leq \delta. $$
\end{proof}

Next, we want to show for minima $V(\e)$ close to $U$, there is an open set around each $V(\e)$ that ``captures" the Jacobi iterates such that they never leave that set.

Here is the intuition behind the proof. Suppose $V(\e)$ is a local minimum. Consider a connected level set $L$ around $V(\e)$. Because our algorithm always decreases the objective function, if we start in $L$ then we shouldn't leave it. The only way we can leave $L$ is if we take a step size large enough to move us far from the local minimum $V(\e)$ to an region where the objective function value is smaller than in $L$. However, if we define a set $S$ that is contained in $L$ and in which the step sizes are always sufficiently small, then it is possible to show that the iterates will never leave $S$.

% local minimum vs minimum of \G
% mention what breaks if not unique local min

\begin{lemma}[Convergence ball]
\label{lem:capture}
For all $\gamma > \delta > 0$, there exist $\e_0, r, s > 0$ such that for all $0 \leq \e \leq \e_0$, and for all local minima $V(\e)$ of $F(V,\e)$ on the set $\Gamma = \{V : | V - U | < \gamma\}$ satisfying  $ || U - V(\e) || <  r $, if we start the algorithm at a point $V_k$ in the set
$$ D(V(\e), \e, \delta) = \{ || V - V(\e) || < \delta ;\; F(V,\e) < F(V(\e), \e) + s \}. $$
then we will also have $V_{k+1} \in D(V(\e), \e, \delta)$.
\end{lemma}

\begin{proof}
By \lemmaref{convergence-threshold}, there exists an $\e_0 > 0$ and an $r > 0$ such that for all $0 \leq \e \leq \e_0$ and for $|| V - V(\e) || < r$, where $V(\e)$ is a local minimizer of $F(V,\e)$ satisfying $ || U - V(\e) || <  r $, we have
$$ || V - V(\e) || + || d(V) || < \delta. $$

Let $\phi(t,\e) = \inf_{t < || V - V(\e) || ;\; V \in \Gamma} F(V,\e) - F(V(\e), \e) \geq 0$ and observe that $\phi(t,\e)$ is monotonically increasing in $t$.
Let $s = \inf_{0 \leq \e \leq \e_0} \phi(r, \e)$ and consider the set
$$ D(V(\e), \e, \delta) = \{ || V - V(\e) || < \delta ;\; F(V,\e) < F(V(\e), \e) + s \}. $$
Suppose that $V_k \in D(V(\e), \e, \delta)$. Since
$$ \phi( || V_{k} - V(\e) || ) \leq F(V_k, \e) - F(V(\e), \e) < s \leq \phi(r, \e) $$
and $\phi$ is monotonically increasing, we have $ || V_{k} - V(\e) || < r$, and thus
$ || V_{k+1} - V(\e) || < \delta $. Also, $F(V_{k+1}, \e) \leq F(V_k, \e)$, so
$$ F(V_{k+1}, \e) - F(V(\e), \e) < s. $$
Thus $V_{k+1} \in D(V(\e), \e, \delta)$.
\end{proof}

The next lemma says that for small enough $\e$, most of these ``capture" sets also contain the unperturbed minimizer $U$.

\begin{lemma}[Convergence balls in the vicinity of global optima]
\label{lem:interior}
For all $\gamma \geq \delta \geq 0$, 
there exists an open set $C$ around $U$, 
as well as $\e_0, t > 0$ such that for all $0 \leq \e \leq \e_0$, for all $0 \leq \delta \leq \delta_0$, and for all local minimizers $V(\e)$ such that $|| U - V(\e) || < t$, $C \subseteq D(V(\e), \e, \delta)$.
\end{lemma}

\begin{proof}
Let $\delta > 0$ be fixed. Recall from \lemmaref{capture}, that the sets $D(V(\e), \e, \delta)$ have the form
$$ D(V(\e), \e, \delta) = \{ || V - V(\e) || < \delta ;\; F(V,\e) < F(V(\e), \e) + s \}, $$
where $s$ is a constant independent of $\e$. These sets are defined for all local minima $V(\e)$ such that $|| V(\e) - U || < r$, for some $r > 0$. Let $\e_1$ be the upper bound on $\e$ that is given by the lemma.

Let $t'$ be such that by the uniform continuity of $f$, we have $ | F(U,\e) - F(V(\e),\e) | < s / 4 $ for $|| U - V(\e) || < t'$ and for all $0 \leq \e \leq \e_1$.
Let $\e_2$ be such that for $0 \leq \e, \e' \leq \e_2$, $ || F(V,\e) -  F(V,\e') || < s / 4 $ for all $V$ such that $|| V - U || < \delta$.
Finally let $\e_0 = \min(\e_1, \e_2)$ and let $t = \min(t', r, \delta/2)$.

Define the set $C$ as
$$ C = \{ || V - U || < \delta/2 ;\; F(V,0) < F(U, 0) + s / 4 \}. $$
For $V \in C$ and for $0 \leq \e \leq e_0$, we have
\begin{align*}
| F(V,\e) - F(V(\e),\e) | 
& \leq | F(V,0) - F(V,\e) | + | F(U,\e) - F(V(\e),\e) | \\
& \;\;\;\;\;\;\;\; + | F(U,0) - F(U,\e) |  + | F(V,0) - F(U,0) | \\
& <  s/4 + s/4 + s/4 + s/4 = s.
\end{align*}
Moreover, for $V \in C$,
$$ || V - V(\e) || \leq || V - U || + || U - V(\e) || < \delta / 2 + \delta / 2 = \delta. $$
This establishes that $C \subseteq D(V(\e), \e, \delta)$.
\end{proof}

Thus the sets $D(V(\e), \e, \delta)$ have non-empty interior and the size of that interior is bounded from below. Next, we would like to show that for small enough perturbations, there exist local minima $V(\e)$ of $F(V,\e)$ that are arbitrarily close to $U$.

\begin{lemma}[Existence of close local minima]
\label{lem:perturbed-minimum-is-close}
For all $\gamma > \delta > 0$, there exists an $\e_0 > 0$ such that for $0 \leq \e \leq \e_0$, there is a $V(\e)$ such that $||V(\e) - U|| < \delta$ and $V(\e)$ is a local minimizer of $F(V, \e)$
in the sense that $F(V(\e), \e) \geq F(V, \e)$ on the set $\{ V : || V - V(\e) || < \gamma \}$.
\end{lemma}

\begin{proof}
By compactness, for every $\e$, there exists a minimum $V(\e)$ of $F(V,\e)$ on the set $\{ V : || U - V || \leq \gamma \}$. 
Suppose that the claim of the lemma does not hold; then there is a $\gamma > \delta' > 0$ and a sequence of $V(\e_n), \e_n$ with $\e_n \to 0$ and $\delta' \leq ||V(\e_n) - U|| \leq \gamma$ such that
$$ F(V(\e_n), \e_n) - F(U, \e_n) \leq 0 $$
for all $n$. Taking limits, we find that $F(Y, 0) \leq F(U, 0)$, where $Y = \lim_{n \to \infty} V(\e_n)$ and $\delta' \leq ||Y - U|| \leq \gamma$, contradicting the fact that $U$ was the only minimum on $\Gamma$.
\end{proof}

The next lemma deals with the initializer $W(\e)$.


\begin{lemma}[Diagonalization of a single matrix]
\label{lem:diagonalize-one-matrix}
Suppose the eigenvalues of the $\sM_0$ are distinct. Let $\e > 0$, and let $W(\e)$ be the estimate of the eigenvalues obtained by diagonalizing one of the $\sM_\e$. As $\e \to 0$, $W(\e) \to U$.
\end{lemma}

\begin{proof}
Follows from the fact that eigenvectors and eigenvalues of $M + \e D$ are continuous in $\e$ for small enough $\e$ \cite{lax1997linear}.
\end{proof}

We use all of the above results to establish the following important lemma says that we can converge arbitrarily close to a global optimum for small amounts of noise.

\begin{lemma}[Convergence to vicinity of global minimum]
There exist $\delta_0 > 0$ and $\e_0 > 0$ such that for all $0 \leq \delta < \delta_0$, there exists an $0 \leq \e < \e_0$ such that when the Jacobi algorithm is initialized at a point $W(\e)$ obtained from diagonalizing one matrix will almost surely converge to a local minimum $V$ of $F(\cdot, \sM_\e)$ with $|| V - U || < 2 \delta$.
\end{lemma}

\begin{proof}

By \lemmaref{interior}, 
for all $\gamma \geq \delta \geq 0$, 
there exists an open set $C$ around $U$, 
as well as $\e_1, t > 0$ such that for all $0 \leq \e \leq \e_1$, for all $0 \leq \delta \leq \delta_0$, and for all local minimizers $V(\e)$ such that $|| U - V(\e) || < t$, $C \subseteq D(V(\e), \e, \delta)$, where $D(V(\e), \e, \delta)$ is a set defined in \lemmaref{capture}.

Let one such $\delta > 0$ be fixed. By \lemmaref{perturbed-minimum-is-close}, there exists an $\e_2 > 0$ such that for $0 < \e \leq \e_2$, there exists a local minimizer $V(\e)$ such that $||V(\e) - U|| < \min(t,\delta)$.

Now let $\beta > 0$ be the radius of a ball around $U$ that is contained in $C$. 
By \lemmaref{diagonalize-one-matrix}, there exists an $\e_3 > 0$ such that for $0 < \e \leq \e_3$, $||W(\e) - U|| < \beta$. Note that the lemma holds because we obtain eigenvalues by random projection, and hence they will be distinct almost surely.

Since $||W(\e) - U|| < \beta$, $W(\e) \in C$. Suppose that we start the algorithm on the function $F(V,\e)$ at $W(\e)$. Then since $S \subseteq D(V(\e),\e,\delta)$, all subsequent iterates will be in $D(V(\e),\e,\delta)$ as well. By compactness, the iterates will converge to a point $Y$ satisfying $|| V(\e) - Y || < \delta$. Furthermore, since $|| U - V(\e) || < \min(t,\delta)$, we have
$$|| U - Y || < 2\delta.$$
Thus the lemma holds with $\delta_0 := \gamma$ and $\e_0 = \min(\e_1, \e_2, \e_3)$.

\end{proof}

\subsection{Cardoso's lemma holds in a neighborhood of $U$}

Finally, we will make the argument that Cardoso's lemma holds for the points to which the Jacobi method will converge.

First, recall that any orthogonal matrix $V$ can be written as $U\exp(E)$ for some skew-symmetric matrix $E$.
The fact that $V = (I+E)U + o(E)$ follows from this observation by using the series form of the matrix exponential $\exp(E)$.

Cardoso's result holds for any $V = (I+\e E')U + o(\e E')$, where $E = O(1)$. Thus, it is enough to show that the $E$ defined above satisfies $E = O(\e)$. To prove this, we will use the following lemma by Cardoso:

\begin{lemma}[Cardoso]
\label{lem:cardoso-foc}
If $V$ is critical point of $F(\cdot, \sM)$, then
$S(V, \sM) = S^T(V,\sM),$
where
$$S(V, \sM) := \sum_k\sum_{i\neq j} (e_i^T V^T M_k V e_j)(e_i e_j^T V^T M_k^T V - V^TM_k^T V e_ie_j^T)$$
\end{lemma}

\begin{lemma}
Let $V = (I+E)U + o(E)$ be the expanded expression of a local minimizer $V(\e)$ of $F(\cdot, \sM_\e)$. Then $|| E || = O(\e)$ as $\e \to 0$.
\end{lemma}

\begin{proof}

Before we proceed, observe that the faction that $V$ converges to a global minimizer $U$ by our previous lemma and thus $E \to 0$ as $\e \to 0$. All we need to establish is the rate. For this, we will use Lemma \ref{lem:cardoso-foc}. Recall that $V$ is a critical point of $F$ whenever $S(V, \sM) = S(V, \sM)^T$, where
$$S(V, \sM) := \sum_k\sum_{i\neq j} (e_i^T V^T M_k V e_j)(e_i e_j^T V^T M_k^T V - V^TM_k^T V e_ie_j^T).$$

It is shown by Cardoso (1994) that
$$(S(V, \sM_\e) - S(V, \sM_\e)^T)_{ij} = 2 \e \sum_k (d_i (k) - d_j(k)) e_i^T U^T R_k U e_j + 2 E_{ij} \sum_k (d_i(k) - d_j(k))^2 + o(\e) + o(E_{ij}). $$
Thus, we can define 
$$ f_{ij}(E_{ij}, \e) = (S(V, \sM_\e) - S(V, \sM_\e)^T)_{ij}. $$
Let $e_n$ be any sequence such that $V(e_n) \to U$ as $e_n \to 0$ and let $E_{ij}^{(n)}$ be the $(i,j)$-th element of the matrix $E_n$ defined in $V_n = (I + E_n) + o(E_n)$.
Combining this with Cardoso's expansion and using the fact that $V(e_{(n)})$ is a minimizer, we have that
$$0 = A_{ij} E_{ij}^{(n)} + B_{ij} \e_n + o(E_{ij}) + o(\e), $$
for all $n$, where $A_{ij}$ and $B_{ij}$ are the constants from Cardoso's expansion. This immediately establishes that $E_{ij} = O(\e)$ (with constant $B_{ij}/A_{ij}$). The fact that $||E|| = O(\e)$ follows by combining the result for each $(i,j)$.

\end{proof}

The above lemma establishes that Lemma \ref{lem:cardoso-1} to holds for points attained by the Jacobi algorithm. 

\begin{corollary}
For small enough $\e > 0$, the bounds in Theorems \ref{thm:ortho-fact-plugin} and \ref{thm:ortho-fact-random} hold almost surely for the output of our orthogonal tensor diagonalization procedure.
\end{corollary}


==> theory.tex <==
%DEPRECATED
% AC: This is a merger of the ortho and non-ortho sections
\section{Theoretical Guarantees}
\label{sec:theory}

Let us now look at the theoretical properties of \algorithmref{joint}.
We will now focus on the orthogonal setting; we return to discuss the
non-orthogonal setting towards the end of the section.

\paragraph{Convergence}
\ac{@VC: Please include content here}

\paragraph{Robustness}

Assured that \algorithmref{joint} converges to a global optimum even in
presence of noise, the next natural step is to ask how sensitive the
global optima of $F(V)$ are to noise. For the ease of exposition, we
restrict ourselves to symmetric third-order orthogonal tensors: $T
= \sum_{i=1}^k \pi_i v_i^{\otimes 3}$. The proofs for this section can
be found ing \appendixref{ortho-proofs}.

Our sensitivity analysis builds on the following perturbation analysis result for
the simultaneous diagonalization of matrices in
\citet{cardoso1994perturbation}:
\begin{lemma}[Orthogonal joint diagonalization perturbation]
  \label{lem:cardoso}
  \ac{Reword to assume that $M_i$ are random projections of $T$}. 
  Let $M_1, \dots, M_L$ be a set of simultaneously diagonalizable
  symmetric matrices formed by the random projection of $T$, with eigenvectors $V$, and let $\hat M_l = M_l + \e R_l$ for $l \in
  [L]$ be
  perturbed versions of the same, where each $R_l$ has unit operator
  norm.
  A minimizer $\Vt$ of \equationref{objective} is
  of the form
  \begin{align*}
    \Vt &= V(I + \e E) + o(\e),
  \end{align*}
  where $E \in \mathbb R^{d \times d}$ is a skew-symmetric matrix with
  zeros on the diagonal. For $i \neq j$,
  \begin{align*}
  E_{ij} &= \frac{\sum_{l=1}^L (\lambda_{il} - \lambda_{jl})  v_i^\top R_l v_j}{\sum_{l=1}^L (\lambda_{il} - \lambda_{jl})^2},
  \end{align*}
  where $\lambda_{il}$ is the $i$-th eigenvalue of matrix $M_l$.
\end{lemma}

\lemmaref{cardoso} tells us that while the estimated eigenvectors $\Vt$
are still sensitive to the eigengaps of the projected matrices,  the error in recovering
eigenvector $v_i$ will approximately depend on the ``average eigengap'' over all the
matrices:
% In particular, the error in recovering
%eigenvector $v_i$ depends on the ``average eigengap'' over all the
%matrices, 
\begin{align*}
  \|\vt_i - v_i\|_2^2 &\sim \max_{j \neq i} \frac1L \sum_{l=1}^L \frac{1}{(\lambda_{il} - \lambda_{jl})}. 
\end{align*}
In our case, the matrices $M_l \eqdef T(I,I,w_l) = \sum_{i} \pi_i (v_i^\top w_l) v_i
v_i^\top$ that we are diagonalizing are projections of a tensor $T$ along vectors $\{w_l\}_{l=1}^L$; we can control their eigenvalues through our choice of $w_l$.
\lemmaref{cardoso} suggests that a good way of choosing the $\{w_l\}_{l=1}^L$ is to
ensure that the projected eigengap is bounded away from zero for at
least one $M_l$. 

One way of ensuring this is to project along the true eigenvectors $v_i$: then at least one matrix will have a large eigengap and the error term $E_{ij}$ will be bounded. Of course, the true $v_i$ are unknown, but we can do almost as well by either using ``plugin" estimates of the $v_i$, or by using many random projections. We formalize these two claims in the theorems below.

%Before we proceed, let us expose some structure shared across the matrices $(M_l)$.
%Firstly, note that
%$\lambda_{il} - \lambda_{jl} = w_l^\top (\pi_i v_i - \pi_j v_j)$. Let
%$p_{ij} \eqdef \pi_i v_i - \pi_j v_j$ so that the eigengap is simply
%$w_l^\top p_{ij}$. Furthermore, let $r_{ij} \eqdef R(v_i, v_j, I)$\footnote{Note that $r_{ij} = r_{ji}$ because $R$ is symmetric.} so that
%$ v_i^\top R_{l} v_j = R(v_i, v_j, w_l) = r_{ij}^\top w_l$.
%The expression for $E_{ij}$ can be rewritten as:
%\begin{align*}
%  E_{ij} &= \frac{\sum_{l=1}^L w_l^\top p_{ij} r_{ij}^\top w_l}
%  {\sum_{l=1}^L w_l^\top p_{ij} p_{ij}^\top w_l}.
%\end{align*}

% Although the perturbation is still sensitive to the eigengap, the eigengap is in a sense averaged across the multiple matrices. For example, observe that if the eigengap $|\lambda_{il} - \lambda{jl}|$ is small for some $i, j, l$, then it will play almost no role in $E_{ij}$. Similarly, as $\min_{l, l'} |\lambda_{il} - \lambda{jl}| / |\lambda_{il'} - \lambda{jl'}| \to 0$, $E_{ik} \to \max_{l} 1 / |\lambda_{il} - \lambda{jl}|$. Thus may bad eigengaps may not affect the error.

\paragraph{Plugin projections}
If the $w_l$ are
approximately the eigenvectors $v_i$, then $w_l^\top (\pi_i
v_i - \pi_j v_j) \approx \pi_i \delta_{il}$: there is some projection
such that the eigengap between $v_i$ and $v_j$ is atleast $\pi_i$.
With this choice, 
the perturbation on the $v_i$ no longer dependens on the eigengap of the diagonalized matrices.
%\begin{lemma}[Diagonalization error with plug-in projections]
%  %\label{lem:e-ij-plugin}
%Let $w_1, \ldots, w_k$ be approximations of $v_1, \ldots, v_k$: $\|w_l - v_l\|_2 \le \gamma$,
%  and let $\sMh = \{\Mh_1, \ldots, \Mh_L\}$ be constructed via
%  projection of $\Th$ along $w_1, \ldots, w_L$.
%If the set of matrices $\sMh$ is simultaneously diagonalized, then the
%  first-order error $E_{ij}$ is bounded from above:
%\begin{align*}
%  E_{ij} &\le \frac{ p_{ij}^\top r_{ij}}{\|p_{ij}\|^2} + O(\gamma).
%\end{align*}
%\end{lemma}

%When the approximation is on the same order as the perturbation, i.e.
%$\gamma \le C\e$, then we find that we recover the eigenvectors $v_i$
%well and with no dependence on the eigengap.
\begin{theorem}[Tensor factorization with plugin projections]
  \label{thm:ortho-fact-plugin}
  Let $w_1, \ldots, w_k$ be approximations of $v_1, \ldots, v_k$: $\|w_l - v_l\|_2 \le \gamma \le C\e$, for some constant $C$,
    and let $\sMh = \{\Mh_1, \ldots, \Mh_k\}$ be constructed via
    projection of $\Th$ along $w_1, \ldots, w_k$.
  Then,
  \begin{align*}
    \| \vt_i - v_i \|_2 
    &\leq 
    \frac{\sqrt{\|\pi\|_1 \pi_{\max}}}{\pi_{\min}^2} \e 
     + o(\e).
  \end{align*}
\end{theorem}

\paragraph{Random projections}

Of course, we do not have access to the eigenvectors or even
approximations of them a priori. 
However, it turns out that by choosing a small number of random projections, we can again ensure that
the $E_{ij}$ are bounded with high probability such that there is again no dependence on the eigengap.
%We will now show that this is indeed the case. 
% First, we show that each element $(E_{ij})$ is bounded with high
% probability,
% \begin{lemma}[Concentration of diagonalization errors]
%   \label{lem:e-ij-conc-1}
% Let $w_1, \ldots, w_L$ be i.i.d.~random Gaussian vectors, $w_l \sim
%   \sN(0, I)$, and let $\sMh = \{\Mh_1, \ldots,
%   \Mh_L\}$ be constructed via projection of $\Th$ along $w_1, \ldots,
%   w_L$.
% Further, assume $L \ge 16\log(2\delta)^2$. 
% Then, with probability at least $1 - \delta$, 
% \begin{align*}
%     E_{ij} 
%         &\le
%         \frac{p_{ij}^\top r_{ij}}{\|p_{ij}\|_2^2} 
%             + \frac{10 \log(2/\delta)}{\sqrt L} \frac{\|r_{ij} \|_2}{\|p_{ij}\|_2}.
% \end{align*}
% \end{lemma}
% This leads to the following bound on the errors in the eigenvectors themselves.
\begin{theorem}[Tensor factorization with random projections]
  \label{thm:ortho-fact-random}
  Let $w_1, \ldots, w_L$ be i.i.d.~random Gaussian vectors, $w_l \sim
    \sN(0, I)$, and let $\sMh = \{\Mh_1, \ldots,
    \Mh_L\}$ be constructed via projection of $\Th$ along $w_1, \ldots,
    w_L$.
  Furthermore, let $L \ge 16 \log(2 k (k-1)/\delta)^2$, then, with probability at least $1-\delta$,
  \begin{align*}
    \| \vt_i - v_i \|_2 
      &\leq 
      \frac{2\sqrt{\|\pi\|_1 \pi_{\max}}}{\pi_{\min}^2} \e 
      + 10\sqrt{2} \log(2k(k-1)/\delta) \frac{\sqrt{k/L}}{\pi_{\min}} \e 
        + o(\e),
  \end{align*}
  for all $i \in [d]$.
\end{theorem}

\theoremref{ortho-fact-random} says that with $O(k)$ random
projections, we can recover the eigenvectors
$v_i$ with about the same precision as if we used approximate
eigenvectors, with high probability.
Moreover, as $L \to \infty$, there is no gap between the precision of
the two methods. The error of both approaches depends on $||\pi||_1$,
which can potentially grow as $O(k)$; however, in several applications,
particularly in the method of moments,  $\pi$ is a vector of
probabilities and therefore $||\pi|||_1$ is a constant.

\paragraph{Non-orthogonal}

\begin{itemize}
  \item State that we do not have guarantees that we will converge to
    local optima using Q1RD. However, in practice, local optima are quite rare.
  \item We can also show that the global optima are sorta-kinda robust
    to noise.
\end{itemize}

\begin{theorem}[Non-orthogonal tensor factorization with random projections]
  \label{thm:non-ortho-random}
  Let $w_1, \ldots, w_L$ be i.i.d.~random Gaussian vectors, $w_l \sim
    \sN(0, I)$, and let $\sMh = \{\Mh_1, \ldots,
    \Mh_L\}$ be constructed via projection of $\Th$ along $w_1, \ldots,
    w_L$.
  Assume incoherence $\mu$: $v_i^\top v_j \le \mu$ for $i \neq j$.
  Furthermore, let $L \ge \left(\frac{50 \log(15 k (k-1)/\delta)}{1-\mu^2}\right)^2$, then, with probability at least $1-\delta$,
   \begin{align*}
    \|\vt_j - v_j\|_2 
    &\le \frac{4 |\pi_{\max}|}{\pi_{\min}^2 (1 - \mu^2)} 
      \left(
      \sqrt{(4 + \mu(d-1)) \|\pi\|_1 \pi_{\max}} + \left( 20 + \sqrt{L_0} \right) \log(15/\delta)\sqrt{d/L}
      \right).
  \end{align*}
\end{theorem}

